InSpectre: Breaking and Fixing Microarchitectural Vulnerabilities by Formal Analysis

The recent Spectre attacks has demonstrated the fundamental insecurity of current computer microarchitecture. The attacks use features like pipelining, out-of-order and speculation to extract arbitrary information about the memory contents of a process. A comprehensive formal microarchitectural model capable of representing the forms of out-of-order and speculative behavior that can meaningfully be implemented in a high performance pipelined architecture has not yet emerged. Such a model would be very useful, as it would allow the existence and non-existence of vulnerabilities, and soundness of countermeasures to be formally established. In this paper we present such a model targeting single core processors. The model is intentionally very general and provides an infrastructure to define models of real CPUs. It incorporates microarchitectural features that underpin all known Spectre vulnerabilities. We use the model to elucidate the security of existing and new vulnerabilities, as well as to formally analyze the effectiveness of proposed countermeasures. Specifically, we discover three new (potential) vulnerabilities, including a new variant of Spectre v4, a vulnerability on speculative fetching, and a vulnerability on out-of-order execution, and analyze the effectiveness of three existing countermeasures: constant time, Retpoline, and ARM's Speculative Store Bypass Safe (SSBS).

==> app-list-examples.tex <==
\section{List of examples}\label{exs}
\noindent\textbf{Example~\ref{example:1}: }\stylecode{$r_1$ := $r_1$+$1$}\\
  \begin{center}
\begin{tikzpicture}[node distance=2.3cm,auto,>=latex']

\pomsetstyle                      
\picexp{t_1}{\top}{r_1}
\picload[right of=t_1]{t_2}{\top}{\Regs}{t_1}
\picexp[right of=t_2]{t_3}{\top}{t_2+1}
\picstore[right of=t_3]{t_4}{\top}{\Regs}{t_1}{t_3}

\picload[below = \pomsetnewline of t_2]{t_5}{\top}{\Pc}{}
\picexp[right of=t_5]{t_6}{\top}{t_5+6}
\picstore[right of=t_6]{t_7}{\top}{\Pc}{}{t_6}

\draw[->]  (t_1) edge (t_2) (t_2) edge (t_3) (t_3) edge (t_4);
\draw[->]  (t_5) edge (t_6) (t_6) edge (t_7);
\end{tikzpicture}
\end{center}

\noindent\textbf{Example~\ref{example:branch}: }\stylecode{beq a}\\
\begin{center}
\begin{tikzpicture}[node distance=2.5cm,auto,>=latex']

  \pomsetstyle

  \picloadT{t_1}{\Regs}{z}
  \picexpT[right of=t_1]{t_2}{t_1 = 1}
  \picloadT[right of=t_2]{t_3}{\Pc}{}
  \picstore[below = \pomsetnewline of t_1]{t_4}{t_2}{\Pc}{}{a}
  \picstore[below = \pomsetnewline of t_3]{t_5}{\neg t_2}{\Pc}{}{t_3+4}

 \draw[->]
 (t_1) edge (t_2)
 (t_2) edge (t_4)
 (t_2) edge (t_5) (t_3) edge (t_5);

\end{tikzpicture} 
\end{center}

\noindent\textbf{Example~\ref{example:active-store}: }\stylecode{*(1):=1; *(0):=0; *(1):=3; *(1);}\\
  \begin{center}
\begin{tikzpicture}[node distance=4cm,auto,>=latex']

\pomsetstyle
  
% \tikzset{res/.style={ellipse,draw,minimum height=0.5cm,minimum width=0.8cm}}


                      
\node[pblock,label={$t_{11}$},name=a1]{$1$};                      


\node[pblock,label={$t_{12}$},name=a2, right of = a1]{$\store{\Locs}{t_{11}}{1}$};                      


\node[pblock,label={[xshift=-.2cm]$t_{21}$},name=a3,  below  = \pomsetnewline of a1]{$0$};                      

\node[pblock,label={[xshift=-.2cm]$t_{22}$},name=a4, right of=a3 ]{$\store{\Locs}{t_{21}}{2}$};                      

\node[pblock,label={[xshift=-.2cm]$t_{31}$},name=a5,  below  = \pomsetnewline of a3]{$1$};                      

\node[pblock,label={[xshift=-.2cm]$t_{32}$},name=a6, right of=a5 ]{$\store{\Locs}{t_{31}}{3}$}; 

\node[pblock,label={[xshift=-.2cm]$t_{41}$},name=a7,  below  = \pomsetnewline of a5]{$1$};                      

\node[pblock,label={[yshift=-0.4cm, xshift=1.0cm]$t_{42}$},name=a8, right of=a7 ]{$\load{\Locs}{t_{41}}$}; 

\draw[->]  (a1) edge (a2) (a3) edge (a4) (a5) edge (a6) (a7) edge (a8);

% \node[draw,dashed,ellipse,fit = (a2)(a6), above = .3cm of a8] {};
% \node[draw,rectangle,minimum width=3.2cm,minimum height=3cm,fit = (a2)(a6)] {};
% \node[draw,dashed,minimum width=2.5cm,minimum height=2cm,rectangle,fit = (a4)(a6)] {};
% \node[draw,dotted,rectangle,minimum width=1.5cm,minimum height=1.2cm,fit = (a6)] {};


\end{tikzpicture}
  \end{center}

\noindent\textbf{Example~\ref{example:spectre:v2}: }\stylecode{*p:=\&f; (*p)()}\\
\begin{center}
\begin{tikzpicture}[node distance=3cm,auto,>=latex']
\pomsetstyle
\node[name=a'_1]{$a_1$};
\picstoreT[right =.3cm of a'_1]{t_{11}}{\Locs}{p}{\&f}
\picstoreT[right of = t_{11}]{t_{12}}{\Pc}{}{a_2}
\node[name=a'_2,below =\pomsetnewline of a'_1]{$a_2$};
\picloadT[right =.3cm of a'_2]{t_{21}}{\Locs}{p}
\picexpT[right of = t_{21}]{t_{22}}{t_{21}}
\picstoreT[right of = t_{22}]{t_{23}}{\Pc}{}{t_{22}}
\draw[->]  (t_{21}) edge (t_{22}) ;
\draw[->]  (t_{22}) edge (t_{23}) ;
\end{tikzpicture}
\end{center}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ccs2020-main"
%%% End:


==> app-sec-condition.tex <==
\section{Security Condition}\label{app:ni}
Alternatively, we can define the security condition directly on the target model, in the style of standard noninterference.

\begin{definition}[Noninterference]
 Let $P$ be a program with transition relation $\singlestep{}{}$, and
 $\sim_P$ a security policy. $P$ satisfies noninterference iff for all
 $\newstate_1, \newstate_2 \in \conf $ such that $\newstate_1 \sim_P
 \newstate_2$  
 and $\pi_1 = \newstate_1 \singlestep{}{}  \cdots$, 
 there exists an execution  $\pi_2 = \newstate_2 \singlestep{}{}  \cdots$ and $\trace(\pi_1) = \trace(\pi_2)$.
 
\end{definition}

Noninterference ensures that if the observations do not enable an attacker 
to refine his knowledge  of sensitive information beyond what is allowed by the policy $\sim_P$,  the program can be considered secure.
%
Noninterference can accommodate partial release of sensitive information by refining definition of indistignuishability relation $\sim_P$. 
In our context, a precise definition of $\sim_P$ can be challenging to define. 
However,  we ultimately aim at showing that the OOO/speculative model does not leak more information than the in-order (sequential) model, thus  
capturing the intuition that microarchitectural features like OOO and speculation do not introduce additional leaks. 

Therefore, instead of defining the policy $\sim_P$ explicitly, we split it in two relations $\sim$ (as in Def.~\ref{def:ci}) and $\sim_D$, where the former models information of the initial state that 
is known by the attacker, i.e., the public resources,  and the latter models information that the attacker is allowed to learn during the  execution via observations. Hence, $\sim_P = \sim \cap \sim_D$. 
This characterization allows for a simpler formulation of the security condition that is transparent on the definition of $\sim_D$, as described in Def.~\ref{def:ci}. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ccs2020-main"
%%% End:


==> proof-correct-ooo.tex <==
\section{Proof Memory Consistency}
To prove consistency we demonstrate a reorder theorem. We first
formalize when an out-of-order execution is ordered:
Let $\pi = \sigma \step{\vec l}{}^\ast \sigma'$ be an partial out of
order trace, $\pi$ is ordered iff for every $i < j$,
$\modifiedname{\pi[i], \pi[i+1]} \leq \modifiedname{\pi[j],
  \pi[j+1]}$.

Several auxiliary lemmas.
\begin{lemma}
  \label{lemma:storage-eq-eval}
  if $\forall t \in n(e) . \storage(t) = \storage'(t)$ then
  $\storage[e]=\storage'[e]$
\end{lemma}
\begin{proof}~\todo{Move to axioms!}
  Proof is trivial
\end{proof}

\begin{lemma}
  \label{lemma:step}
If $\state  = (I, \storage, \commits, \decodes) \step{}{} (I', \storage',
\commits', \decodes') = \state'$, let $t=\modifiedname{\state
  \step{}{} \state'}$ then exist
$I'', v$ such that
\begin{itemize}
\item $I' = I \cup I''$ and  $n(I) < n(I'')$ and $I' \neq I
  \Rightarrow t = \decodedname{\state \step{}{} \state'}$.
\item $\storage = \storage'$ or $\storage' = \storage \cup \{t \mapsto v\}$ and $t = \executedname{\state \step{}{} \state'}$.
\item $\commits = \commits'$ or $\commits' = \commits \cup \{t\}$ and  $t = \committedname{\state \step{}{} \state'}$.
\item $\decodes = \decodes'$ or $\decodes' = \decodes \cup \{t\}$ and  $t = \executedname{\state \step{}{} \state'}$.
\end{itemize}
\end{lemma}
\begin{proof}
  Proof should be trivial by induction over the transition rules
\end{proof}


\begin{lemma}\label{lemma:pas:eq}
  if $n(I') \geq t$ and $dom(\storage') \geq t$ then
  $t_{lst} = LST(\pars{I}{\storage}{t}{\restype}{a}) = LST(\pars{I
    \cup I'}{\storage \cup \storage'}{t}{\restype}{a})$
  and $t_{lst} < t$.
\end{lemma}
\begin{proof}
   $\prs{I \cup I'}{t}{\restype} =
   \{\ass{c}{t'}{\store{\restype}{e_1}{e_2}} \in I \cup I' \mid t' <
   t\} =
   \prs{I}{t}{\restype}
   \cup
   \{\ass{c}{t'}{\store{\restype}{e_1}{e_2}} \in I' \mid t' <   t\}
   $ ($n(I) \geq t$) $ = \prs{I}{t}{\restype}$ (1).
   
   $\pars{I \cup I'}{\storage \cup \storage'}{t}{\restype}{a} =
   \{\ass{c}{t'}{\store{\restype}{e_1}{e_2}} \in \prs{I \cup I'}{t}{\restype}
   \mid
   ((\storage \cup \storage')[c] \vee (\storage \cup \storage')[c] = \bot) \wedge
   ((\storage \cup \storage')[e_1] = a \vee (\storage \cup
   \storage')[e_1] = \bot)\} = $ \\
   by (1) $\{\ass{c}{t'}{\store{\restype}{e_1}{e_2}} \in \prs{I}{t}{\restype}
   \mid
   ((\storage \cup \storage')[c] \vee (\storage \cup \storage')[c] = \bot) \wedge
   ((\storage \cup \storage')[e_1] = a \vee (\storage \cup
   \storage')[e_1] = \bot)\}$

   For all $\ass{c}{t'}{\store{\restype}{e_1}{e_2}} \in
   \prs{I}{t}{\restype}$, $t' < t$. Therefore, by
   Axiom~\ref{axiom:tranpilation}, $n(c) < t' < t$ and $n(e_1) < t' < t$.
   By Lemma~\ref{lemma:storage-eq-eval} we have
   $(\storage \cup \storage')[c] = \storage[c]$ and
   $(\storage \cup \storage')[e_1] = \storage[e_1]$.
\end{proof}

The reorder theorem establishes that for any out of order partial
trace $\rho = \sigma \step{\vec l}{}^\ast \sigma'$  exists an ordered
trace $\pi = \sigma \step{\vec l'}{}^\ast \sigma'$.
\todo{plus things on the order of memory stores}

The proof is done by induction over the length of partial traces and
relies on the following shift lemma~\ref{lemma:switch}.


\begin{lemma}\label{lemma:switch-pre}
If $\sigma \step{l_1}{} \sigma_1 \step{l_2}{} \sigma_2$ and
$\modifiedname{\sigma_1 \step{l_2}{} \sigma_2} <
\modifiedname{\sigma \step{l_1}{} \sigma_1}$.
Let  $I_1 = I \cup I_{t_1}$,
  $\storage_1 = \storage \cup \storage_{t_1}$,
  $\commits_1 = \commits \cup \commits_{t_1}$,
  $\decodes_1 = \decodes \cup \decodes_{t_1}$ and
  $I_2 = I_1 \cup I_{t_2}$,
  $\storage_2 = \storage_1 \cup \storage_{t_2}$,
  $\commits_2 = \commits_1 \cup \commits_{t_2}$,
  $\decodes_2 = \decodes_1 \cup \decodes_{t_2}$.
And
  Let $I' = I \cup I_{t_2}$,
  $\storage' = \storage \cup \storage_{t_2}$,
  $\commits' = \commits \cup \commits_{t_2}$,
  $\decodes' = \decodes \cup \decodes_{t_2}$.
Then $\sigma \step{l_2}{} \sigma'$ and
 $\modifiedname{\sigma \step{l_2}{} \sigma'} =
 \modifiedname{\sigma_1 \step{l_2}{} \sigma_2}$.
\end{lemma}
\begin{proof}
  First, if $\modifiedname{\sigma \step{l_2}{} \sigma'} = t_2$ then
  $\ass{c}{t_2}{o} \in I_1$. By lemma~\ref{lemma:step} $n(I_{t_1}) > n(I)$. Since
  $\modifiedname{\sigma \step{l_2}{} \sigma'} = t_1 > t_2$, and $t_1
  \in n(I)$ then $n(I_1) > t_2$. Therefore $\ass{c_2}{t_2}{o_2} \in I$
  (0).
  The same lemma also guarantees that
  $dom(\storage_{t_1}) \subseteq \{t_1\}$, $\commits_{t_1} \subseteq
  \{t_1\}$, and $\decodes_{t_1} \subseteq \{t_1\}$.
  
  Proof is done by case over the transition rules.

  \paragraph{Case exec expression}
  In this case $o = \expr$. By rule $exp$ we have
  $\storage_1(t_2) = \perp$,  $\storage_1[c]$, and $v=\storage_1[e]$.
  Also, $\storage_{t_2} = \{t_2 \mapsto v\}$,
  $\commits_{t_2}=\emptyset$, $\decodes_{t_2}=\emptyset$, and
  $I_{t_2} = \emptyset$ (1).

  By Axiom\ref{axiom:tranpilation}.3, $n(c) < t_2 < t_1$ and $n(e) < t_2 <
  t_1$ (2). By (1,2) and Lemma~\ref{lemma:storage-eq-eval} we have that
  $\storage[c]$ and $v=\storage[e]$
  (3).

  By (1) we have that   $\storage(t_2) = \perp$ (4).
  
  Using rule $exp$ and (0, 3, 4) we have that 
  $\sigma \step{}{} (I, \storage \cup \{t_2 \mapsto v\}, \commits,
  \decodes) = \state'$.


  \paragraph{Case exec store}
  In this case $o_2 = \store{\restype}{e_a}{e_v}$. By rule $store$ we
  have
  $\storage_1(t_2) = \perp$,  $\storage_1[c]$, $v=\storage_11[e_v]$, 
  $a=\storage_1[e_a]$.
  Also, $\storage_{t_2} = \{t_2 \mapsto v\}$,
  $\commits_{t_2}=\emptyset$, $\decodes_{t_2}=\emptyset$, and
  $I_{t_2} = \emptyset$ (1).
  
By \ref{axiom:tranpilation}.3, $n(c) < t_2 < t_1$, $n(e_v) < t_2 <
  t_1$, and $n(e_a) < t_2 <  t_1$ (2). By (1,2) and Lemma~\ref{lemma:storage-eq-eval} we have that
  $\storage[c]$, $v=\storage[e_v]$, and $a=\storage[e_a]$  (3).

  By (1) we have that   $\storage(t_2) = \perp$ (4).
  
  Using rule $store$ and (0, 3, 4) we have that 
  $\sigma \step{}{} (I, \storage \cup \{t_2 \mapsto v\}, \commits,
  \decodes) = \state'$.

  \paragraph{Case exec load}
  In this case $o_2 = \load{\restype}{e_a}$. By rule $load$ we
  have
  $\storage_1(t_2) = \perp$,  $\storage_1[c]$, $a=\storage_1[e_a]$.
  Moreover, $t_{lst} = LST(\pars{I_1}{\storage_1}{t_2}{\restype}{a})$
and $v=\storage_1(t_{lst})$.
  Also, $\storage_{t_2} = \{t_2 \mapsto v\}$,
  $\commits_{t_2}=\emptyset$, $\decodes_{t_2}=\emptyset$, and
  $I_{t_2} = \emptyset$ (1).
  
  By \ref{axiom:tranpilation}.3, $n(c) < t_2 < t_1$
  and $n(e_a) < t_2 <  t_1$ (2). By (1,2) and Lemma~\ref{lemma:storage-eq-eval} we have that
  $\storage[c]$ and $a=\storage[e_a]$  (3).

  By (1) we have that   $\storage(t_2) = \perp$ (4).

  By Lemma~\ref{lemma:pas:eq} we have $t_{lst} =
  LST(\pars{I}{\storage}{t_2}{\restype}{a})$. (5)
  
  Since $t_{lst} < t_2 \leq t_1$ and (1) we have
  $\storage(t_{lst})=v$. (6)
  

  By (0, 3,4,5,6) and rule $load$ we have
  $\sigma \step{}{} (I, \storage \cup \{t_2 \mapsto v\}, \commits,
  \decodes) = \state'$.

  \todo{However, here we must dead with the label, which may differ}

  \paragraph{Case commit}
  In this case $o_2 = \store{\Locs}{e_a}{e_v}$. By rule $commit$ we
  have
  $\storage_1(t_2) = v$, $t_2 \not \in \commits_1$, 
  $\storage_1[e_a] = a$,
  $t_{lst} = LST(\pars{I_1}{\storage_1}{t_2}{\Locs}{a})$,
  and $t_{lst} \in \commits_1$.
  Also, $\storage_{t_2} = \emptyset$,
  $\commits_{t_2}= \{t_2\}$, $\decodes_{t_2}=\emptyset$, and
  $I_{t_2} = \emptyset$ (1).

  As usual, by \ref{axiom:tranpilation}.3, $n(c) < t_2 < t_1$ and $n(e_a) < t_2 <  t_1$ (2). By (1,2) and Lemma~\ref{lemma:storage-eq-eval} we have that
  $\storage[c]$ and $a=\storage[e_a]$  (3).

  By (1) and $t_2 < t_1$ we have that   $\storage(t_2) = v$ and $t_2
  \not \in \commits$ (4)

  By Lemma~\ref{lemma:pas:eq} we have $t_{lst} =
  LST(\pars{I}{\storage}{t_2}{\Locs}{a})$. (5)

  Since by (1)  $t_{lst} \in \commits_1$, by (Hyp)  $\commits_1 =
  \commits \cup \commits_{t_1}$, by (0) $\commits_{t_1} \subseteq
  \{t_1\}$, $t_{lst} < t_2 < t_1$, then $t_{lst} \in \commits$ (6)

  By (0, 3,4,5,6) and rule $commit$ we have
  $\sigma \step{}{} (I, \storage, \commits \cup \{t_2\},
  \decodes) = \state'$.
  
  \paragraph{Case fetch}
  In this case $o_2 = \store{PC}{e_a}{e_v}$. By rule $fetch$ we
  have
  $\storage_1(t_2) = v$, $t_2 \not \in \decodes_1$, 
  $\storage_1[e_a] = a$,
  $t_{lst} = LST(\pars{I_1}{\storage_1}{t_2}{PC}{a})$,
  and $t_{lst} \in \decodes_1$.
  Also, $\storage_{t_2} = \emptyset$,
  $\commits_{t_2}= \emptyset$, $\decodes_{t_2}=\{t_1\}$, and
  $I_{t_2} = TR[v]$, and $n(I_{t_2}) > n(I) \cup n(I_{t_1})$ (1).

  As usual, by \ref{axiom:tranpilation}.3, $n(c) < t_2 < t_1$ and $n(e_a) < t_2 <  t_1$ (2). By (1,2) and Lemma~\ref{lemma:storage-eq-eval} we have that
  $\storage[c]$ and $a=\storage[e_a]$  (3).

  By (1) and $t_2 < t_1$ we have that   $\storage(t_2) = v$ and $t_2
  \not \in \decodes$ (4)

  By Lemma~\ref{lemma:pas:eq} we have $t_{lst} =
  LST(\pars{I}{\storage}{t_2}{PC}{a})$. (5)

  We must prove that 
  (a) $t_{lst} \in \decodes$,
  and (b) $I = I_1$. The last one is needed to guarantee that the
  names of $TR_{n(I)}[v]$ are the same of $TR_{n(I_1)}[v]$: i.e., that
  we decode in order.


  For (a),  Since by (1)  $t_{lst} \in \decodes_1$, by (Hyp)  $\decodes_1 =
  \decodes \cup \decodes_{t_1}$, by (0) $\decodes_{t_1} \subseteq
  \{t_1\}$, $t_{lst} < t_2 < t_1$, then $t_{lst} \in \decodes$ (6)

  For (b) we have that if $I_1 \neq I$, then $I_{t_1} \neq \emptyset$
  and by Lemma~\ref{lemma:step} $t_1 = \decodedname{\sigma \step{}{}
    \sigma_1}$.
  \todo{This part must be completed} This means that $t_1$ was decoded
  in the previous step. However, this contradicts the
  invariant~\ref{lem:invariant} that decodes are done in order.
  Therefore $I_1 = I$ and $TR_{n(I)}[v] = TR_{n(I_1)}[v]$ (7)

  By (0, 3,4,5,6,7) and rule $decode$ we have
  $\sigma \step{}{} (I \cup I_{t_2}, \storage, \commits,
  \decodes \cup \{t_2\}) = \state'$.
\end{proof}


\begin{lemma}\label{lemma:pas:mono}
  if $\state \step{}{} \state'$, $t \in n(I)$, $t_{lst} =
  LST(\pars{I}{\storage}{t}{\restype}{a})$ and $\storage(t_{lst})
  \neq \perp$ then $LST(\pars{I'}{\storage'}{t}{\restype}{a}) = t_{lst}$.
\end{lemma}
\begin{proof}
  Let $p = \{ \ass{c}{t'}{\store{\restype}{e_a}{e_v}} \in I \mid
  t_{lst} \leq t' < t\}$.
 By Lemma~\ref{lemma:step}, $I' = I \cup \bar I$ and $n(\bar I)
 > n(I)$.
Therefore,
$p = \{ \ass{c}{t'}{\store{\restype}{e_a}{e_v}} \in I' \mid  t_{lst}
\leq t' < t\}$ (1).

Since $t_{lst} =  LST(\pars{I'}{\storage'}{t}{\restype}{a})$, then for
every $\ass{c}{t'}{\store{\restype}{e_a}{e_v}} \in p$ such that $t' >
t_{lst}$ holds:
(2a) $\storage[c] = false$ or (2b) $\storage[e_a]\neq q$.

 Since $\storage[c] \neq \perp$ and $\storage[\expr_a] \neq \perp$ then
  their value cannot be updated in $\storage'$ and by lemma~\ref{lemma:storage-eq-eval} we have that
  $\storage'[c]$ or $a \neq \storage'[\expr_a]$  (3).

For the last store, the other hand, we have
$\ass{c_{lst}}{t_{lst}}{\store{\restype}{e_{lst, a}{e_{lst,v}}}} \in
  p$ and 
  $(\storage[c_{lst}]=\perp \vee \storage[c_{lst}])$ or
  $(\storage[e_{lst,a}]=\perp \vee a = \storage[e_{lst,a}])$ (4).
  
  By Lemma~\ref{lemma:invariant:store} we have that if a store is
  executed, then its condition and address are defined: i.e.,
  Since $\storage(t_{lst}) = v$ then $\storage[c_{lst}]$ and
  $\storage[e_{lst,a}] \neq perp$.
  Therefore these values cannot be updated in $\storage'$ and by lemma~\ref{lemma:storage-eq-eval} we have that
  $\storage'[c_{lst}]$ and
  $\storage'[e_{lst,a}] = a$  (5).

  (3) and (5) implies $t_{lst} =
  LST(\pars{I'}{\storage'}{t}{\restype}{a})$.
  
\end{proof}

\begin{lemma}
  \label{lemma:switch}
If $\sigma \step{l_1}{} \sigma_1 \step{l_2}{} \sigma_2$ and
$\modifiedname{\sigma_1 \step{l_2}{} \sigma_2} <
 \modifiedname{\sigma \step{l_1}{} \sigma_1}$ then exists $\state'$
 such that
 $\sigma \step{l_2}{} \sigma' \step{l_1}{} \sigma_2$ and
 $\modifiedname{\sigma' \step{l_1}{} \sigma_2} \geq
 \modifiedname{\sigma \step{l_2}{} \sigma'}$.
\end{lemma}
\begin{proof}
  Let $t_1 = \modifiedname{\sigma \step{l_1}{} \sigma_1}$ and $t_2 = \modifiedname{\sigma_1 \step{l_2}{} \sigma_2}$.
  By Lemma~\ref{lemma:step}, we have that
  $I_1 = I \cup I_{t_1}$,
  $\storage_1 = \storage \cup \storage_{t_1}$,
  $\commits_1 = \commits \cup \commits_{t_1}$,
  $\decodes_1 = \decodes \cup \decodes_{t_1}$ and
  $I_2 = I_1 \cup I_{t_2}$,
  $\storage_2 = \storage_1 \cup \storage_{t_2}$,
  $\commits_2 = \commits_1 \cup \commits_{t_2}$,
  $\decodes_2 = \decodes_1 \cup \decodes_{t_2}$.

  Let $I' = I \cup I_{t_2}$,
  $\storage' = \storage \cup \storage_{t_2}$,
  $\commits' = \commits \cup \commits_{t_2}$,
  $\decodes' = \decodes \cup \decodes_{t_2}$.
  The first transition is proven by Lemma~\ref{lemma:switch-pre}.
  For the second transition we work by cases on the transition rules:

  \paragraph{Case exec expression}
  By rule $exp$ we have
  $\ass{c}{t_1}{\expr} \in I$,
  $\storage(t_1) = \perp$,  $\storage[c]$, and $v=\storage[\expr]$.
  Also, $\storage_{t_1} = \{t_1 \mapsto v\}$,
  $\commits_{t_1}=\emptyset$, $\decodes_{t_1}=\emptyset$, and
  $I_{t_1} = \emptyset$ (1).

  If $\sigma_{t_2} = \emptyset$ then $\storage'(t_1) = \perp$,
  $\storage'[c]$, and $v=\storage'[\expr]$ (2).
  Otherwise, $\storage_{t_2} = \{ t_2 \mapsto v_2\}$ for some $v_2$. In
  this case, $\storage(t_2) = \perp$, due to
  invariant~\ref{lemma:invariant}.
  Therefore $\storage'(t_1) = \perp$.
  Since $\storage[c] \neq \perp$ and $\storage[\expr] \neq \perp$ then
  $t_2 \not \in n(c) \cup n(\exp)$ and by lemma~\ref{lemma:storage-eq-eval} we have that
  $\storage'[c]$ and $v=\storage'[\expr]$.  (2).
  
  Using rule $exp$ and (1, 2, 3) we have that 
  $\sigma' \step{}{} (I', \storage' \cup \{t_1 \mapsto v\}, \commits',
  \decodes') = \state_2$.

  \paragraph{Case exec store}
  By rule $store$ we have
  $\ass{c}{t_1}{\store{\restype}{e_a}{e_v}} \in I$,
  $\storage(t_1) = \perp$,  $\storage[c]$, $v=\storage[\expr_v]$, and $a=\storage[\expr_a]$.
  Also, $\storage_{t_1} = \{t_1 \mapsto v\}$,
  $\commits_{t_1}=\emptyset$, $\decodes_{t_1}=\emptyset$, and
  $I_{t_1} = \emptyset$ (1).

  If $\sigma_{t_2} = \emptyset$ then $\storage'(t_1) = \perp$,
  $\storage'[c]$, $v=\storage'[\expr_v]$, and $v=\storage'[\expr_a]$ (2).
  Otherwise, $\storage_{t_2} = \{ t_2 \mapsto v_2\}$ for some $v_2$. In
  this case, $\storage(t_2) = \perp$, due to invariant~\ref{lemma:invariant}. 
  Therefore $\storage'(t_1) = \perp$.
  Since $\storage[c] \neq \perp$,  $\storage[\expr_v] \neq \perp$, and $\storage[\expr_a] \neq \perp$ then
  $t_2 \not \in n(c) \cup n(\exp_v) \cup n(\exp_a)$ and by lemma~\ref{lemma:storage-eq-eval} we have that
  $\storage'[c]$, $v=\storage'[\expr_v]$, $a=\storage'[\expr_a]$  (2).
  
  Using rule $store$ and (1, 2, 3) we have that 
  $\sigma' \step{}{} (I', \storage' \cup \{t_1 \mapsto v\}, \commits',
  \decodes') = \state_2$.

  \paragraph{Case exec load}
  By rule $load$ we have
  $\ass{c}{t_1}{\load{\restype}{e_a}} \in I$,
  $\storage(t_1) = \perp$,  $\storage[c]$, $a=\storage[\expr_a]$.
  Moreover,
  $t_{lst} = LST(\pars{I}{\storage}{t_1}{\restype}{a})$
and $v=\storage(t_{lst})$.
  Also, $\storage_{t_1} = \{t_1 \mapsto v\}$,
  $\commits_{t_1}=\emptyset$, $\decodes_{t_1}=\emptyset$, and
  $I_{t_1} = \emptyset$ (1).

  As usual,
  If $\sigma_{t_2} = \emptyset$ then $\storage'(t_1) = \perp$,
  $\storage'[c]$, and $v=\storage'[\expr_a]$ (2).
  Otherwise, $\storage_{t_2} = \{ t_2 \mapsto v_2\}$ for some $v_2$. In
  this case, $\storage(t_2) = \perp$, due to invariant~\ref{lemma:invariant}. 
  Therefore $\storage'(t_1) = \perp$.
  Since $\storage[c] \neq \perp$ and $\storage[\expr_a] \neq \perp$ then
  $t_2 \not \in n(c) \cup n(\exp_a)$ and by lemma~\ref{lemma:storage-eq-eval} we have that
  $\storage'[c]$, $a=\storage'[\expr_a]$  (2).

  We cannot prove that $\pars{I}{\storage}{t_1}{\restype}{a} =
  \pars{I \cup I_{t_2}}{\storage \cup I_{t_2}}{t_1}{\restype}{a})$,
  since $t_2 < t_1$. Two things could happen . (a) $t_2$ may decode new
  stores (i.e. $I_{t_2} \neq emptyset$). However, these new stores
  have names greater than $t_2$, therefore they do not affect
  $\pars{I}{\storage}{t_1}{\restype}{a}$.
  Alternatively, (b) $t_2$ may make defined the evaluation of the
  condition or expression of a store. In this case, we must show that
  $PAS$ can only decrease that that the last element remain unchanged
  once its value has been set in $\storage$.
  In fact, Lemma~\ref{lemma:pas:mono} guarantees that
  $LST(\pars{I'}{\storage'}{t_1}{\restype}{a}) = t_{lst}$ (3)

  Also $\storage'(t_{lst}) = v$ (4).

  Finally from (2,3,4) and rule $load$ we have that 
  $\sigma' \step{}{} (I', \storage' \cup \{t_1 \mapsto v\}, \commits',
  \decodes') = \state_2$
  \todo{again: label can differ}

  \paragraph{Case commit}
  By rule $commit$ we have
  $\ass{c}{t_1}{\store{\Locs}{e_a}{e_v}} \in I$,
  $\storage(t_1) = v$, $t_1 \not \in \commits$, 
  $\storage[e_a] = a$,
  $t_{lst} = LST(\pars{I}{\storage}{t_1}{\Locs}{a})$,
  and $t_{lst} \in \commits$.
  Also, $\storage_{t_1} = \emptyset$,
  $\commits_{t_1}= \{t_1\}$, $\decodes_{t_1}=\emptyset$, and
  $I_{t_1} = \emptyset$ (1).

  As usual, we have using lemma~\ref{lemma:storage-eq-eval} that
  $\storage'(t_1) = v$
  $\storage'[c]$, $a=\storage'[\expr_a]$  (2).
  and  $t_{lst} \in \commits'$ (3).

  Lemma~\ref{lemma:pas:mono} guarantees that
  $LST(\pars{I'}{\storage'}{t_1}{\Locs}{a}) = t_{lst}$ (4)

  We must guarantee that $t_1 \not \in \commits'$: i.e. $t_1 \not \in
  \commits_{t_2}$.

  If $t_1 \in  \commits_{t_2}$ then, by Lemma~\ref{lemma:step} $t_2 =
  t_1$ and the second transition has been committed $t_1$. This is not
  possible, since $t_1 \in \commits_1$, therefore $\sigma_1 \step{}{}
  \sigma_2$ cannot commit $t_1$.
  Therefore $t_1 \not \in \commits'$ (5).

   Finally from (2,3,4,5) and rule $commit$ we have that 
  $\sigma' \step{}{} (I', \storage', \commits' \cup \{t_1\},
  \decodes') = \state_2$

  \paragraph{Case fetch}
  By rule $fetch$ we have
  $\ass{c}{t_1}{\store{PC}{e_a}{e_v}} \in I$,
  $\storage(t_1) = v$, $t_1 \not \in \decodes$, 
  $\storage[e_a] = a$,
  $t_{lst} = LST(\pars{I}{\storage}{t_1}{PC}{a})$,
  and $t_{lst} \in \decodes$.
  Also, $\storage_{t_1} = \emptyset$,
  $\commits_{t_1}= \emptyset$, $\decodes_{t_1}= \{t_1\}$, and
  $I_{t_1} = TR_{n(I)}[v]$ (1).

  As usual, we have using lemma~\ref{lemma:storage-eq-eval} that
  $\storage'(t_1) = v$
  $\storage'[c]$, $a=\storage'[\expr_a]$  (2).
  and  $t_{lst} \in \decodes'$ (3).

  Lemma~\ref{lemma:pas:mono} guarantees that 
  $LST(\pars{I'}{\storage'}{t_1}{PC}{a}) = t_{lst}$ (4)

  We must guarantee that $t_1 \not \in \decodes'$: i.e. $t_1 \not \in
  \decodes_{t_2}$. This is relatively simple: since $t_2$ is a decode
  then $t_2 \not \in \decodes_1$ and $t_2 \not \in \decodes$
  Since $t_2 < t_1$, 
  then $t_2 \in \pars{I}{\storage}{t_1}{PC}{a})$. However, this
  contradicts the fact that $t_{lst} \in \decodes$ \todo{Probably we
    must show an invariant that decodes are done in order}.
  Therefore $I_{t_2} = \emptyset$
  and $t_1 \not \in \decodes'$ (5).

   Finally from (2,3,4,5) and rule $fetch$ we have that 
  $\sigma' \step{}{} (I' \cup  TR_{n(I')}[v], \storage', \commits',
  \decodes' \cup \{t_1\}) = (I \cup  TR_{n(I)}[v], \storage', \commits',
  \decodes' \cup \{t_1\}) = \state_2$
  
\end{proof}

\begin{theorem}
 Out of order semantics implies memory consistency.
\end{theorem}
\begin{proof}
 It follows from Lemma~\ref{lemma:switch-pre} and Lemma~\ref{lemma:switch}.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "model"
%%% End:


==> proof-spec-consistency-short.tex <==


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "sp2020"
%%% End:


==> security-ooo.tex <==
\section{Security OOO}
The security goal should be something like this:
For every program $p$, for every initial states $\state_1$ and
$\state_2$ such that the sequential traces $\pi_1$ and $\pi_2$ are
indistinguishable \todo{partial traces}, for every partial out-of-order trace $\rho_1$
starting from $\state_1$, exists an
out-of-order trace $\rho_2$ starting from $\state_2$ that is
indistinguishable from $\rho_1$.

\begin{definition}[Security Condition]
\label{def:security}
 
\end{definition}


In general this is not possible, see the example in
Section~\ref{sec:attack:ooo}.
Also, in some cases this is even not desirable. Take again the same
example, where the flag $Z$ is already public. There is no reason to
prevent the channel introduced by reordering.

The initial idea was to ``synthetize'' a relation $R$ that must be
satisfied by all indistinguishable sequential traces  $\pi_1$ and
$\pi_2$ that entails the security goal. This allows us to lift
verification of the out-of-order model to a more tractable in-order
model. In the next step, it can be verified that low-equivalence
of the initial states entails (if some countermeasure is applied) the
relation for in-order executions.
The initial candidate for this relation was the following:
\begin{itemize}
  \item without restriction on reordering (i.e. infinite store buffers,
    pipeline with infinite size) reordering of two assignment happens
    iff dependencies of the second assignment do not depend on the
    first assignment.
  \item so the relation should entails that given two observable
    assignments $\iota_1$ and $\iota_2$ of $\pi_1$ and the
    two observable assignments $\iota'_1$ and $\iota'_2$ of $\pi_2$
    (these assignments exist because the two traces are
    indistinguishable), $\iota_1$ depends $\iota_2$ iff $\iota'_1$ depends $\iota'_2$.
  \item things get a bit complicated because the dependencies evolve
    during the execution. The idea was that dependencies are all names
    that $\iota_1$ must waits before execution. Since names affect
    conditions and address of stores, this set is reduced while
    executing, since we discover that some memory stores cannot affect
    the address used by $\iota_1$ or that some stores should not be
    executed at all.
  \item these dependencies should be monotone, and the $\iota_1$
    should fire only after all its dependency have been executed.
  \item Unfortunately things are more complicated due to conditional
    stores. $\iota_1$ may wait a store having condition $c$ and
    address $e$. In this case $\iota_1$ must waits all names in $c$
    and $e$. However, as soon as $c$ is evaluated to false (or $e$ is
    evaluated to an address different that the address of $\iota_1$),
    $\iota_1$ can fire, without waiting the dependencies of $e$ (or
    the dependencies of $c$). This is due to a sort of short circuit
    rule and makes the story more complicated, since in two
    indistinguishable runs $\iota_1$ and $\iota'_1$ may have different
    dependencies but fire at the same time.
\end{itemize}

For these reason we decide for a simpler approach: prove that constant
time is secure. However, we cannot simply rely on constant time at
binary level, since security depends on how microcode is executed.
We phrase constant time as follows:
\begin{definition}
  \label{def:ct}
  A program is constant time if for every pair states $\state_1 =_L
  \state_2$ that are low-equivalent, for every in-order  partial executions of
  $n$ transitions $\state_1 \step{}{}^n \state$ and $\state_2
  \step{}{}^n \state'$ the following properties hold
  \begin{itemize}
  \item $I = I'$, $\commits=\commits'$, $\decodes=\decodes'$:
    the same instructions are put in flight (one can be
    a bit less restrictive, requiring that there is a bijection among
    names.)
  \item if $\ass{c}{t}{o} \in I$ then $\sigma[c] = \sigma'[c]$
    and $(\storage(t) = \perp) \Leftrightarrow (\storage'(t) = \perp)$
    \begin{itemize}
      \item if $o = \load{\Locs}{e}$ then $\sigma[e] = \sigma'[e]$
      \item if $o = \store{\restype}{e_1}{e_2}$ then $\sigma[e_1] =
        \sigma'[e_1]$, notice that this is required also for registers
    \end{itemize}
  \end{itemize}
\end{definition}
The big simplification obtained by constant time is that we have the same
instructions in flight, which enables to prove a bisimulation between
the two out-of-order executions.

TODO:
\begin{itemize}
 \item Check related work on CT for machine code
 \item Add example to motivate constant time
 \item CT at microarchitectural level can be insecure (cf. cmove instructions)
 \item Alternatives: cache partitioning, bit masking
\end{itemize}

We first introduce a relation, which is induced by
Definition~\ref{def:ct}.
\begin{definition}
  \label{def:ct}
 $\state \sim \state'$ iff
  \begin{itemize}
  \item $I = I'$, $\commits=\commits'$, $\decodes=\decodes'$
  \item if $\ass{c}{t}{o} \in I$ then $\sigma[c] = \sigma'[c]$
    and $(\storage(t) = \perp) \Leftrightarrow (\storage'(t) = \perp)$
    \begin{itemize}
      \item if $o = \load{\Locs}{e}$ then $\sigma[e] = \sigma'[e]$
      \item if $o = \store{\restype}{e_1}{e_2}$ then $\sigma[e_1] =
        \sigma'[e_1]$
    \end{itemize}
  \end{itemize}
\end{definition}

\begin{theorem}
  If a program satisfies \ref{def:ct} then $\sim$ is a bisimulation.
\end{theorem}
\begin{proof}
  Proof is not by cases on the transition rules.
  Let $\state \step{}{} I \cup I_t, \storage \cup \storage_t, \commits
  \cup \commits_t, \decodes \cup \decodes_t = \state_t$.

  \paragraph{Case exec expression}
    By rule $exp$ we have
    $\ass{c}{t}{\expr} \in I$,
    $\storage(t) = \perp$,  $\storage[c]$, and $v=\storage[\expr]$.
    Also, $\storage_{t} = \{t \mapsto v\}$,
    $\commits_{t}=\emptyset$, $\decodes_{t}=\emptyset$, and
    $I_{t} = \emptyset$ (1).

    By ($\sim$)   $\ass{c}{t}{\expr} \in I'$,
    $\storage'(t) = \perp$,  $\storage'[c]$ (2).
    
    We must prove that $\storage'[e] \neq \perp$. We use the decode
    axiom to infer that $n(e) \subseteq n(I) = n(I')$. \todo{Here
      there is confusion between bounded and free names}
    By ($\sim$), $(\storage(n(e)) = \perp ) \Leftrightarrow
    (\storage'(n(e)) = \perp )$.
    Therefore
    $\state' \step{}{} I' , \storage' \cup \{t \mapsto
    v'\}, \commits', \decodes' = \state'_t$. \todo{Notice that $v'$ can differ
      from $v$}

    We must prove the second condition (the first one is trivial) of
    $\sim$ for
    $ \storage \cup \{t \mapsto  v\}$ and     $ \storage' \cup \{t
    \mapsto  v'\}$. 


    
    Let $\ass{c'}{t'}{o'} \in I$. We first look at the condition $c'$
    \begin{itemize}
      \item
    If $\storage[c'] \neq \perp$ then $t \not \in n(c')$ and
    $(\storage
    \cup \storage_t)[c'] = \storage[c']$. By $\sim$ we have
    $\storage[c']=\storage'[c']$, and since $t \not \in n(c')$ then $
    \storage'[c'] = (\storage' \cup \{t
    \mapsto  v'\})[c']$.
    \item If $(\storage \cup \storage_t)[c] = \perp$ then $n(c') \not
      \subseteq n(\storage \cup \storage_t)$. By $\sim$ we have
      $n(\storage \cup \storage_t) = n(\storage' \cup  \{t
    \mapsto  v'\})$. Therefore $(\storage' \cup  \{t
    \mapsto  v'\})[c'] = \perp$.
  \item Otherwise $(\storage \cup \storage_t)[c] \neq \perp$ and
    $\storage[c] = \perp$. Therefore $t \in n(c')$ and $(\storage' \cup \storage'_t)[c] \neq \perp$.

    To complete the proof we use the $\sim$ property \todo{we must add
    this} that $\state$ and $\state'$ are the $i$-th states of two
  partial out-of-order traces $\rho$ and $\rho'$ that start from two low-equivalent initial states $\state_0$ and
  $\state'_0$. Clearly $\state_t$ and   $\state_t$ are the $i+1$-th
  states of $\rho$ and $\rho'$.
  \todo{We do not have this theorem} Since $\rho[:i+1]$ is a partial
  out-of-order trace, there is a partial trace $\rho_s$ that has
  prefix $\rho[:i+1]$ and whose last state is a sequential state $\state_s$: i.e.
  for every $t'' < t'''$ if $\completed{\state_s}{t'''}$ then
  $\completed{\state_s}{t''}$.
  Due to monotonicity of the state components: $(\storage \cup
  \storage_t)[c] = \storage_s[c]$.
  Also due to the reordering theorem, we know that exists an ordered
  execution $\pi$ of  $\rho_s$ that ends in $\state_s$.  Since
  $\state_s$ is a sequential state then $\pi$ is a prefix of the
  in-order execution.

  With the same reasoning we can prove that $\rho'[:i+1]$ is a prefix
  of a trace $\rho'_S$ which ends in a sequential state $\state'_s$;
  that $\storage'_s[c'] = (\storage' \cup
  \storage'_t)[c]$; that exists an in-order execution  $\pi'$ that
  ends in $\state'_s$.\todo{We must prove that these executions: $\pi$
    and $\pi'$ have the same length}

  We can now use the assumption on Property~\ref{def:ct} to show that 
  $\storage'_s[c'] = \storage_s[c']$.

\end{itemize}
the proof for expressions of loads and stores is similar.

  \paragraph{Case exec store}
  This is totally similar to the case of exec expression.

  \paragraph{Case exec load}
  By rule $load$ we have
  $\ass{c}{t}{\load{\restype}{e_a}} \in I$,
  $\storage(t) = \perp$,  $\storage[c]$, $a=\storage[\expr_a]$.
  Moreover,
  $t_{lst} = LST(\pars{I}{\storage}{t}{\restype}{a})$
and $v=\storage(t_{lst})$.
  Also, $\storage_{t} = \{t \mapsto v\}$,
  $\commits_{t}=\emptyset$, $\decodes_{t}=\emptyset$, and
  $I_{t} = \emptyset$ (1).

  By ($\sim$)   $\ass{c}{t}{\load{\restype}{e_a}} \in I'$,
  $\storage'(t) = \perp$,  $\storage'[c]$ (2).

    We must prove that $\storage'[e_a] = a$ via $\sim$ \todo{We must make the
      proof stronger, requiring that $\sim \Rightarrow \storage'[e_a]
      = \storage[e_a]$ for register too.}.
  

    Now the problem is to show that $t_{lst} = LST(\pars{I'}{\storage'}{t}{\restype}{a})$
    and $\storage'(t_{lst}) \neq \perp$.

    Take the set $S = \{\ass{c'}{t'}{\store{\restype}{e'_a}{e'_v}} \in
    I \mid t_{lst} \leq t' < t \}$. Clearly, by $\sim$,
    $S = \{\ass{c'}{t'}{\store{\restype}{e'_a}{e'_v}} \in
    I' \mid t_{lst} \leq t' < t \}$.

    We focus on $e'_a$, the same reasoning can be done for $c'$.
    Let $\ass{c'}{t'}{\store{\restype}{e'_a}{e'_v}} \in S$.
    By  the decode axiom we know that $n(e'_a) < t$.

    \begin{itemize}
      \item
    if $\storage[e'_a] = \perp$, then $n(e'_a) \not \subseteq
    n(\storage)$. By $\sim$,  $n(\storage) = n(\storage')$, therefore
    $\storage[e'_a] = \perp$
    \item if $\storage[e'_a] \neq \perp$ then by $\sim$ we have that
      $\storage[e'_a] = \storage'[e'_a]$
    \end{itemize}
    Therefore $t_{lst} = LST(\pars{I'}{\storage'}{t}{\restype}{a})$.
    Finally, by $\sim$ we have that $\exists v' . \storage'(t_{lst}) =
    v'$.
    
    By applying rule $load$
    $\state' \step{}{} I' , \storage' \cup \{t \mapsto
    v'\}, \commits', \decodes' = \state'_t$. \todo{Notice that $v'$ can differ
      from $v$}

    The other part of the proof is similar to the case of exec expression.

      \paragraph{Case commit}
  By rule $commit$ we have
  $\ass{c}{t}{\store{\Locs}{e_a}{e_v}} \in I$,
  $\storage(t) = v$, $t \not \in \commits$, 
  $\storage[e_a] = a$,
  $t_{lst} = LST(\pars{I}{\storage}{t}{\Locs}{a})$,
  and $t_{lst} \in \commits$.
  Also, $\storage_{t} = \emptyset$,
  $\commits_{t}= \{t\}$, $\decodes_{t}=\emptyset$, and
  $I_{t} = \emptyset$ (1).
  
  By ($\sim$)   $\ass{c}{t}{\store{\Locs}{e_a}{e_v}} \in I$,
  $\exists v' . \storage'(t) = v'$, $t \not \in \commits'$, 
  $\storage'[e_a] = a$,  $\storage'[c]$ (2).

  To show that $t_{lst} = LST(\pars{I'}{\storage'}{t}{\restype}{a})$
  we use the same strategy of case $load$.

  By $\sim$ holds $t_{lst} \in \commits'$.
  Therefore, by applying rule $store$
    $\state' \step{}{} I' , \storage', \commits' \cup \{t\}, \decodes'
    = \state'_t$. \todo{How about labels?}
    
    \paragraph{Case decode}
    It is similar to the case commit. Maybe we must add the condition
    that we update the pc with the same value. This is probably free
    by knowing that the sequential model had the same instructions in flight.
    
  \end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "model"
%%% End:


==> speculation.tex <==
\newcommand{\spec}{\delta}
\newcommand{\newspec}[4]{EXT(#1, #2, #3, #4)}
\newcommand{\specPars}[6]{SPAS(#1, #2, #3, #4, #5, #6)}
\section{Speculation}
We extend the state with a speculation map $\spec: \ANames
\rightharpoonup \Stores$. We also use a set $g$ to keep track for the names that have been speculated. We choose to speculate values of expressions and loads; no speculative guesses on stores. 
Finally, we assume that the parameters to stores and loads are just names (no expressions).
In practice the speculation map keeps track
of the speculative state of names used to compute an instruction.
We introduce the following functions
\todo{Remember that to support speculative execution of fetches, we
  must extend existing mapping for $t$}
\[
  \newspec{\storage}{\spec}{t}{T} = \spec \cup \{t
  \rightarrow  \{t' \rightarrow \storage(t') . t' \in T \cap \dom{\spec}\}\}
\]
\[
\specPars{I}{\storage}{t}{t'}{\restype}{a} =
\bigcup_{\ass{c}{t''}{\store{\restype}{e_1}{e_2}} \in I \land t' \leq t''
   < t}\{
 n(e_1) \cup n(c)
 \}
\]

% \todo{What about condition c?}
\[
\mbox{\sc Expr}\ 
\begin{array}{c}
  \storage(t) = \perp\ \qquad
  \ass{c}{t}{\expr} \in I \qquad \storage[c] \qquad v=\storage[e] \qquad t \in g
  \\ \hline
  I, \storage,\spec \step{}{} \storage\{v/t\},
  \newspec{\storage}{\spec}{t}{n(e) \cup n(c)}
\end{array}
\
\]
\[
\mbox{\sc Store}\
\begin{array}{c}
  \storage(t) = \perp\ \qquad
\ass{c}{t}{\store{\restype}{e_a}{e_v}} \in I \qquad \storage[c] \qquad
  a=\storage[e_a] \qquad v=\storage[e_v] \qquad t \in g
  \\ \hline
  I, \storage, \spec \step{}{×} \storage\{v/t\},
    \newspec{\storage}{\spec}{t}{n(e_a) \cup n(e_v) \cup n(c)}
\end{array}
\
\]
\[
\mbox{\sc Load}\
\begin{array}{c}
  \storage(t) = \perp\ \qquad
\ass{c}{t}{\load{\restype}{e}} \in I \qquad \storage[c] \qquad
  a=\storage[e] \qquad t \in g\\
  \qquad {t_{lst} = LST(\pars{I}{\storage}{t}{\restype}{a})} \qquad v=\storage(t_{lst}) 
  \\ \hline
I, \storage, \commits, \spec \step{(t_{lst} \in \commits \land
  \restype = \Locs) \; ? \;
  \load{\restype}{a} \; : \; \epsilon}{×} \storage\{v/t\},
   \newspec{\storage}{\spec}{t}{n(e) \cup n(c) \cup \{t_{lst}\} \cup \specPars{I}{\storage}{t}{t_{lst}}{\restype}{a}}
\end{array}
\
\]
\[
\mbox{\sc Mem-Commit}\
\begin{array}{c}
  \storage(t) = v \qquad  t \not \in \commits \qquad
\ass{c}{t}{\store{\Locs}{e_a}{e_v}} \in I \qquad  \storage[e_a] = a\\
  t_{lst} = LST(\pars{I}{\storage}{t}{\Locs}{a})
  \qquad t_{lst} \in \commits \\
  t \not \in \dom{\spec}
  \\ \hline
(I, \storage, \commits, \spec) \step{\store{\Locs}{a}{v}}{×} \commits \cup \{t\}
\end{array}
\]
\[
\mbox{\sc Fetch}\
\begin{array}{c}
    \storage(t) = v \qquad  t \not \in \decodes \qquad
\ass{c}{t}{\store{PC}{0}{e_v}} \in I\\
   t_{lst} = LST(\pars{I}{\storage}{t}{PC}{0} \qquad t_{lst} \in
  \decodes \\
\spec' = \newspec{\storage}{\spec}{t}{\{t_{lst}\} \cup
  \specPars{I}{\storage}{t}{t_{lst}}{PC}{0}}\\
  \hline
(I, \storage, \decodes) \step{\store{PC}{0}{v}}{×} I \cup TR[v],
  \decodes \cup \{t\},
  \newspec{\storage}{
   \spec'
  }{n(TR[v])}{\{t\}}
\end{array}
\
\]
\[
\mbox{\sc Commit-ex}\
\begin{array}{c}
  \storage' = \spec(t) \qquad
   \ass{c}{t}{\expr} \in I \qquad
  \dom{\storage'} \cap \dom{\spec} = \emptyset \\ \qquad
  \forall t' \in \dom{\storage'} . \storage(t') = \storage'(t') \qquad t \not\in g
  \\
  \hline
I, \storage, \spec \step{}{×} \spec \setminus \{t \rightarrow \spec(t)\}
\end{array}
\
\]
\[
\mbox{\sc Rollback-ex}\
\begin{array}{c}
  \storage' = \spec(t) \qquad
   \ass{c}{t}{\expr} \in I \qquad
  \exists t' \in \dom{\storage'} . \storage(t') \neq \storage'(t')
  \\
  \hline
  \storage, \spec \step{}{×} \storage \setminus \{t \rightarrow \storage(t)\},
  \spec \setminus \{t \rightarrow \spec(t)\}
\end{array}
\
\]

\[
\mbox{\sc Commit- store no pc}\
\begin{array}{c}
  \storage' = \spec(t) \qquad
  \ass{c}{t}{\store{\restype}{e_a}{e_v}} \qquad
  \restype \neq PC \\
  \dom{\storage'} \cap \dom{\spec} = \emptyset \qquad
  \forall t' \in \dom{\storage'} . \storage(t') = \storage'(t')
  \\
  \hline
I, \storage, \spec \step{}{×} \spec \setminus \{t \rightarrow \spec(t)\}
\end{array}
\
\]
\[
\mbox{\sc Rollback-store no pc}\
\begin{array}{c}
  \storage' = \spec(t) \qquad
  \ass{c}{t}{\store{\restype}{e_a}{e_v}} \qquad
  \restype \neq PC \\
  \exists t' \in \dom{\storage'} . \storage(t') \neq \storage'(t')
  \\
  \hline
  \storage, \spec \step{}{×} \storage \setminus \{t \rightarrow \storage(t)\},
  \spec \setminus \{t \rightarrow \spec(t)\}
\end{array}
\
\]


\[
\mbox{\sc Commit- store PC}\
\begin{array}{c}
  \storage' = \spec(t) \qquad
  \ass{c}{t}{\store{PC}{e_a}{e_v}} \\
  \dom{\storage'} \cap \dom{\spec} = \emptyset \qquad
  \forall t' \in \dom{\storage'} . \storage(t') = \storage'(t')
  \\
  \hline
I, \storage, \spec \step{}{×} \spec \setminus \{t \rightarrow \spec(t)\}
\end{array}
\
\]
\[
\mbox{\sc PC Rollback}\
\begin{array}{c}
  \ass{c}{t}{\store{PC}{0}{e_v}} \in I \qquad
  \storage' = \spec(t) \qquad
  \exists t' \in \dom{\storage'} . \storage(t') \neq \storage'(t')
  \\
  \hline
  I, \storage, \decodes, \spec \step{}{×}
  I \setminus{\spec \downarrow_t}, 
  \storage \setminus \{t\} \setminus{\spec \downarrow_t}, \decodes \setminus \{t\}\setminus{\spec \downarrow_t},  \spec \setminus \{t\}\setminus{\spec \downarrow_t}
\end{array}
\
\]
Notice that fetch can generate several new specs, one for each
transpiled assignment.
\[
\mbox{\sc Commit-load}\
\begin{array}{c}
  \storage' = \spec(t) \qquad
    \ass{c}{t}{\load{\restype}{e_a}} \in I \qquad
  \dom{\storage'} \cap \dom{\spec} = \emptyset \\
  t_{lst} = LST(\pars{I}{\storage'}{t}{\restype}{a}) = LST(\pars{I}{\storage}{t}{\restype}{a})\\
  \forall t' \in \{t_{lst}\} \cup n(e_a) . \storage(t') = \storage'(t')
  \\
  \hline
I, \storage, \spec \step{}{×} \spec \setminus \{t \rightarrow \spec(t)\}
\end{array}
\
\]
\[
\mbox{\sc Rollback-ex}\
\begin{array}{c}
  \storage' = \spec(t) \qquad
  \ass{c}{t}{\load{\restype}{e_a}} \in I \\
  {t_{lst} = LST(\pars{I}{\storage'}{t}{\restype}{a})}\\
  \exists t' \in \{t_{lst}\} \cup n(e_a) . \storage(t') \neq
  \storage'(t')
  \vee
  {t_{lst} \neq LST(\pars{I}{\storage}{t}{\restype}{a})}
  \\
  \hline
  \storage, \spec \step{}{×} \storage \setminus \{t \rightarrow \storage(t)\},
  \spec \setminus \{t \rightarrow \spec(t)\}
\end{array}
\
\]


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "model"
%%% End:

